Monitoring Model Deterioration with Explainable Uncertainty Estimation via Non-parametric Bootstrap

Monitoring machine learning models once they are deployed is challenging. It is even more challenging to decide when to retrain models in real-case scenarios when labeled data is beyond reach, and monitoring performance metrics becomes unfeasible. In this work, we use non-parametric bootstrapped uncertainty estimates and SHAP values to provide explainable uncertainty estimation as a technique that aims to monitor the deterioration of machine learning models in deployment environments, as well as determine the source of model deterioration when target labels are not available. Classical methods are purely aimed at detecting distribution shift, which can lead to false positives in the sense that the model has not deteriorated despite a shift in the data distribution. To estimate model uncertainty we construct prediction intervals using a novel bootstrap method, which improves upon the work of Kumar & Srivastava (2012). We show that both our model deterioration detection system as well as our uncertainty estimation method achieve better performance than the current state-of-the-art. Finally, we use explainable AI techniques to gain an understanding of the drivers of model deterioration. We release an open source Python package, doubt, which implements our proposed methods, as well as the code used to reproduce our experiments.

==> content/miscellaneous.tex <==
%Recent methods for evaluation of uncertainty estimates and robustness to distributional shift such as the case of Malinin et al \cite{datasetShift}, that aim at facilitating distribution shift benchmarking with the "Weather forecasting" dataset \ref{data:weather}.

%The weather forecasting data is sampled in two different dimensions: $(i)$ time-dependent training set is from September 2018 to April 2019 and test set is from May 2019 to September 2019 $(ii)$ and by type of climate in training set the climates are tropical, dry and mild template and in the test set snow and polar.

%We have the first bench-marked uncertainty detection techniques. Where all (uncertainty estimation and classical statistics) techniques indicate correctly that there exists a distribution shift and non-parametric uncertainty estimation for regression models using bootstrap methods provides a better measurement for model deterioration. Our current approach limitations is that even if we have a better estimate of the model deterioration, we are not able to individually detect which features are causing it. The question now changes to \textit{What is the feature or set of features that are downgrading the model performance?}

%Calculating statistical indicators such as Kolmogorov-Smirnov or the Population Stability Index will only inform how much the features from the train and test differ. This is not necessarily informing on the source of model deterioration.



%The field of interpretable and explainable machine learning has emerged as a way to aid our understanding of the inner workings of a model ~\citep{desiderataECB,ShouldNotTrustMe,doshivelez2017rigorous,guidotti_survey,paco_herrera_xai_taxonomi,exaplaining_explanations_ATI,explainabe_public_policy,explaining_explanations_overview_of_interpretability,xai_concepts,rudin2019stop}.
%This motivation is part of the ``Fair, Accountable and Transparency'' research agenda ~\citep{ntoutsi2020bias,weller2019transparency}.

